A DSL for Defining Feature-Level Quality Constraints and the Aggregation of Evaluation Results in DevOps

Quality requirements typically differ among software features, e.g., due to different usage contexts of the features, different impacts of related quality deficiencies onto overall user satisfaction, or long-term plans of the developing organization. For instance, maintainability requirements might be particularly high for software features which are frequently used or bear strategic value for the developing organization. Also, software features where even the smallest delays are perceived as negative by the user will be subjected to specially tight performance requirements. We defined an operational DSL to define software quality requirements as individual feature-level constraints based on quantitative measures. The DSL provides language elements to define the operationalization of measures from external systems, time series operations, time filters, and the automatic evaluation of these feature-level constraints in DevOps based on comparison operators and threshold values. In addition, quality ratings summarize evaluation results of features on an ordinal grading scheme. Likewise, quality gates use these quality ratings to reflect the fitness of software features or the overall software product using different states. Finally, we show an example based on a widely-adopted secure mobile messaging app that illustrates the interplay of the different DSL elements.

==> Revision1/aggregation_language.tex <==
%!TEX root = manuscript.tex
\label{aggregation_language}
In the frame of the development of the TAICOS DSL we already conducted a case study with practitioners \cite{haindl_specifying_2020} who applied the DSL to formulate feature-level maintainability constraints. One important finding of this case study was the practical need articulated by participants of a formalism to aggregate constraint evaluation results. To address this practical requirement, we extended the TAICOS DSL to support the definition of quality ratings and gates. Thereby, the underlying calculation approach provides for default quality ratings, which are calculated even if they have not been explicitly defined. 

Quality ratings aggregate the evaluation results of feature constraints on the level of interests and interest groups on an ordinal scale. Thereby, concrete fulfillment criteria for each grade on the ordinal scale can be defined. As such, they give a quick overview to external stakeholders about the degree quality-related stakeholder interests are fulfilled. 

Quality gates on the other hand summarize multiple quality ratings to determine whether a software feature or the whole software product meets specific quality criteria to proceed to the next engineering step. This decision is based on concrete pass/fail criteria which are defined using the TAICOS DSL.

\subsection{Grammar and Language Elements} 
Similarly to the previous section, when showing grammar rules for the different language elements we highlight \dslkeyword{<non-terminal symbols>} in brackets and \dslkeyword{terminal symbols} without brackets. In this context the most important language elements are \dslkeyword{<QualityRating>} and \dslkeyword{<QualityGate>}. Further, the \dslkeyword{<ProductQuality>} element allows to define a product-level quality gate and product-wide default quality ratings and gates for all software features and stakeholder interests. 

\subsubsection{Formulation and Calculation of Quality Ratings}
Quality ratings (element \dslkeyword{<QualityRating>}) can be defined for interests, interest groups, and individual software features. Depending on which of these levels a quality rating is defined, we distinguish between \textit{constraint-based} and \textit{interest-based quality ratings}. For both types of quality ratings, the calculated grade of a quality rating can be in the range of A-E, with A the best and E the worst. Listing \ref{lst:qualityratings} shows the general grammar rules for defining quality ratings.

\begin{figure}[h!]
\lstset{style=atg,basicstyle=\footnotesize\ttfamily,caption={Grammar rules for defining quality ratings.},captionpos=b,label=lst:qualityratings}
\begin{lstlisting}
<QualityRating> ::= ratingId ": { " 
  ( ConstraintBasedRating> | <InterestBasedRating> ) 
  { ( ConstraintBasedRating> | <InterestBasedRating> ) } "}" .
<ConstraintBasedRating> ::= ratingVal ":" 
  (noFulfilled "of" totalConstraints) | (percentage "of") 
  "constraints"
  [ "and" 
      ("constraint" contraintId) | 
      ("constraints" contraintId {"," contraintId })
  ] "are fulfilled." .
<InterestBasedRating> ::= "average rating of interests"
  [ interestId "," interestId { "," interestId } ] "." .
ratingVal ::= "A" | "B" | "C" | "D" .
\end{lstlisting}
\end{figure}

Constraint-based ratings (\dslkeyword{<ConstraintBasedRating>}) are calculated based on the number or percentage of fulfilled constraints for an individual stakeholder interest of a software feature. In the definition of the same quality rating one must not switch between specifying the degree of fulfillment as an absolute or relative number. Particularly, in case of only a small total number of constraints, specifying the degree of fulfillment with absolute numbers might be more suitable. On the other hand, as the number of total constraints for a particular interest might vary among different software features, defining the degree of fulfillment with relative percentages is more robust when applying the same quality rating for a particular interest to different software features.

At maximum (but not mandatory) four different grades from A-D with descending degrees of constraint fulfillment can be defined. Also, lower grades must not relax the required degree of fulfillment of higher grades. The grade E does not have to be defined explicitly, as it is automatically generated if none of the other grades are fulfilled. To achieve a particular grade, also the fulfillment of one or more specific constraints (referred to by their names) can be demanded. When calculating the grade for a quality rating, the conditions for the defined grades are evaluated in descending order until the actual degree of constraint fulfillment suffices the conditions of a grade. 
As an example, one could define a quality rating \dslkeyword{A: 4 of 4 constraints are fulfilled. B: 3 of 4 constraints and constraint technicalDebtConstraint \newline are fulfilled.} Thus, for an \dslkeyword{A}  grade, all constraints of the interest for which this quality rating was defined would need to be fulfilled. For a B grade, only 3 of the 4 constraints (one being the \dslkeyword{technicalDebtConstraint}) would need to be fulfilled. In case that this constraint is not fulfilled or less than 3 constraints are fulfilled, the resulting grade would be E, as no more further grades are defined. 

Interest-based ratings (element \dslkeyword{<InterestBasedRating>}) can be defined on two levels: If defined for an interest group (second level), the calculation of the grade takes into account constraint-based quality ratings of subordinate individual interests (first level). Contrarily, if defined on the higher level of a software feature (third level), the calculation of the grade is based on quality ratings of the feature's interest groups (second level) and individual interests (first level). In both cases, the resulting grade is calculated based on the average of either all or only selected subordinate quality ratings. Thus, for this type of quality ratings, no grades and respective constraint fulfillment can be defined, but instead a set of quality ratings as the basis for grade calculation. For calculating the grade, the ordinal grades of the subordinate quality ratings are mapped to integer values (A=1, B=2, C=3, D=4, E=5), the average calculated thereof, the resulting floating point arithmetically rounded to an integer value and mapped back to an ordinal grade. An interest-based quality rating can, e.g., be defined as \dslkeyword{average rating of interests} on a software feature with subordinate quality ratings having been graded with A, C, and D. The resulting grade for the quality rating of the software feature would then be calculated as $(A+C+D)/3 = (1+3+4)/3 = (8/3) = 2.67 \approx 3 = C$.

If no quality rating is explicitly specified, the standard grading scheme for quality ratings is applied to calculate the grades. There is an important distinction between standard and default quality ratings: \textit{Standard quality ratings} cannot be specified explicitly as they are calculated automatically in case no quality rating has been defined for the different aggregation levels by the user. In contrast, \textit{default quality ratings} can optionally be specified to set particular quality ratings as defaults for the different aggregation levels. For (standard) constraint-based quality ratings, the following percentages of constraint fulfillment are defined: A $(>=$95\%), B [80-95\%[, C [65-80\%[, D [50-65\%[, E ($<$50\%). For (standard) interest-based quality ratings, the average grade is calculated from the grades of all subordinate interest groups (for quality ratings of software features) and of all subordinate interests (for quality ratings of interest groups). 

\subsubsection{Formulation and Calculation of Quality Gates}
\label{qualitygates}
Quality gates (element \dslkeyword{<QualityGate>}) summarize multiple quality ratings and can be defined for individual software features or for the whole software product. If quality gates shall be checked they must be explicitly defined, as there is no default calculation scheme similar to quality ratings. 

The DSL provides three states for quality gates: \dslkeyword{pass}, \dslkeyword{warn}, and \dslkeyword{fail}. When defining quality gates (\dslkeyword{<GateDefinition>}), at least the criteria for the \dslkeyword{pass} state must be defined, while the definition of the \dslkeyword{warn} state is optional. The \dslkeyword{fail} state does not need to be specified as it is automatically reached if no other state applies. When evaluating quality gates, the conditions for the \dslkeyword{pass} state are checked first. If the conditions for this state are not fulfilled and yet conditions for the \textit{warn} state are defined, those are checked and upon their fulfillment this is the final state. In case this state is not defined or its conditions also are not fulfilled, the final state of the quality gate is \dslkeyword{fail}. Listing \ref{lst:qualitygates} shows the grammar rules for defining quality gates and their states using the DSL.

\begin{figure}[h!]
\lstset{style=atg,basicstyle=\footnotesize\ttfamily,caption={Grammar rules for defining quality gates.},captionpos=b,label=lst:qualitygates}
\begin{lstlisting}
<QualityGate> ::= gateId : "{ " 
  "pass:" <GateDefinition> "."
  [ "warn:" <GateDefinition> "." ] "}" .
<GateDefinition> ::= "average rating of" 
  ("interests"|"features") [referenceId { "," referenceId }] 
  "is" ratingVal 
  [ "and" 
      ( "interest" | "feature" ) 
      referenceId "is rated" ratingVal 
  ] "." .
referenceId ::= featureId | interestId .
\end{lstlisting}
\end{figure}

In general, the state of a quality gate is calculated from the average of multiple quality ratings, whereby I distinguish between \textit{interest-based gates} and \textit{feature-based gates}. Interest-based gates can be defined for individual software features and take into account quality ratings of an individual feature's subordinate interest groups and interests. Likewise, feature-based gates can be defined on the top level of the software product and take into account quality ratings of the product's software features. Similar to quality ratings, the set of quality ratings of interests and features used for calculating the average can be specified in the definition of the quality gate. Also, a particular quality rating can be demanded for an individual interest or software feature (\dslkeyword{ratingReferenceId}). To fulfill a certain state, the calculated average of the quality ratings must meet the conditions defined for this state. 

For illustration purposes, let assume that the \dslkeyword{video} feature of a fictitious software product is particularly important for the developing organization. Defining an (interest-based) quality gate as \dslkeyword{pass: average rating of interests is B.} and leaving out the optional definition of the \textit{warn} means that an average rating of the feature's quality ratings dropping below B leads to failing this quality gate. Therefore, the definition of the \textit{warn} state is intentionally left out. Further, one could define a (feature-based) quality gate for this software product as \dslkeyword{pass: average rating of features is B. warn: average rating of features is C and feature video is rated B.} Apparently, while for the \textit{warn} state the demanded average of the quality ratings is lower than for the \textit{pass} state, the \dslkeyword{video} feature nonetheless must have a quality rating better than or equal B to fulfill at least the \textit{warn} state.

\subsubsection{Defining Default Quality Ratings and Gates}
The \dslkeyword{<ProductQuality>} element allows to define default quality ratings, default quality gates, and the top-level (feature-based) quality gate for the software product. Defaults prevent redundant specifications and can be defined for 
\begin{itemize}
\item quality gates for software features (interest-based gates)
\item quality ratings for software features (interest-based ratings)
\item quality ratings for interests (constraint- \& interest-based ratings)
\end{itemize}
Depending on whether default quality ratings and gates are defined for the software product, individual features or interests (and groups), different types of quality ratings and gates are applicable. As an example, for software features quality ratings and gates require the subordinate interest-based counterparts for their calculation. On the level of interests, constraint- and interest-based quality ratings can be defined as defaults. The former to calculate quality ratings through constraint fulfillment on interest-level (\dslkeyword{constRatingId}), the latter from quality ratings of multiple subordinate interests of an interest group (\dslkeyword{intrstRatingId}). As the total number of constraints might vary among different interests, for default constraint-based quality ratings the required level of constraint fulfillment shall be described in percentage.

The defaults are applied to all features and interests by the TAICOS DSL parser when instantiating the TAICOS model. However, these defaults can be overridden individually by software features or interests.

==> Revision1/case_study.tex <==
%!TEX root = manuscript.tex
\label{case_study}
\subsection{Software Prototype}
\subsection{Scope and Expressiveness of DSL elements}

==> Revision1/concepts.tex <==
%!TEX root = manuscript.tex
\label{concepts}
\begin{figure*}[h]
\centering
\includegraphics[scale=0.34]{images/sequence.pdf}\caption{Integration of the TAICOS approach in DevOps.\label{fig:taicos_concepts}}
\end{figure*}
\change{integration in devops anhand des sequenz diagrams beschreiben. bezug zur value orientation und dass die metriken aus unterschiedlichen systemen kommen können. die dazu wesentlichen haben wir im IET journal identifiziert. betonen, dass die grauen und hellgrauen komponenten die relation zu dem metamodel herstellen. die einzelnen komponenten beschreiben und womit die in der praxis konkret realisiert werden}
For gaining a better understanding of the TAICOS approach, we give a brief overview of the most important concepts shown in Figure \ref{fig:taicos_concepts}. Our approach introduces the concept of \textit{stakeholder interests} to denote top-level non-functional objectives articulated by stakeholder that must be taken into account by all software features. In general, these stakeholder interests are not limited to technical quality-related objectives, but also comprise business-related objectives of stakeholders towards a software system. In the context of this paper, we concentrate on quality-related stakeholder interests solely. The starting point for applying the approach in a DevOps environment is the (1) TAICOS quality model \cite{haindl_extension_2019} on the upper left part of the figure. This quality model allows to specify the stakeholders' interests as quality requirements on the level of individual software features and is created typically during the \textit{plan} phase of the DevOps cycle. 

The feature-level quality requirements are decomposed and defined using the TAICOS DSL as (2) feature constraints. Constraints are composed of different quantitative measures which are operationalized through instruments. During the \textit{build}, \textit{continuous integration}, \textit{deployment}, and \textit{operation} phase of the DevOps cycle, these measures are acquired from the different systems automatically from software connectors associated with these instruments. For specifying the evaluation of these measures, the TAICOS DSL provides different time filters, time series operations, and comparison operators. In the context of the \textit{continuous feedback} phase of the DevOps cycle, the measures are collected from the different instruments and the fulfillment of the feature constraints evaluated based on these measures. The individual constraint evaluation results are (3) aggregated to facilitate their interpretation in the context of a particular software feature or the overall software product. Thereby, quality ratings summarize multiple constraint evaluation results based on a five-element grading scheme. Quality gates can take three states to reflect the appropriateness of a feature or the overall software product for the next engineering step, e.g., productive deployment, system testing, or feature experimentation \cite{kevic_characterizing_2017,olsson_hypex_2014}, by taking account these quality ratings. The final (4) quality evaluation has two directions: The quantitative evaluation is done automatically through the TAICOS software prototype and takes into account constraint violations and the thereof calculated quality ratings and the status of quality gates. The qualitative evaluation needs to be done manually among the relevant stakeholders of the software project and takes into account the projected feature value for the developing organization and the end user of the software. This evaluation is based on strategic and economic considerations impacting the \textit{software value chain} of a company \cite{wirtz_business_2011,pussep_software_2012} and thus cannot be conducted in an automated fashion. In case of important findings from any of these two directions of evaluation, the TAICOS quality model is adapted accordingly. For instance, by relaxing or enforcing existing feature constraints or by adding new ones to better suit the overall quality-related stakeholder interests.
\change{hier referenz auf das IET journal} \cite{haindl_value-oriented_2021}

==> Revision1/conclusion.tex <==
%!TEX root = manuscript.tex
\label{conclusion}
This paper presented an operational DSL for expressing feature-level quality requirements and the aggregation of evaluation results for individual software features and the overall software product. In this context, \textit{operational} refers to defining these quality requirements in a manner that allows their automated evaluation of fulfillment and the aggregation of these results in DevOps. Our DSL allows to define these quality requirements individually for each software feature as feature constraints, which are based on quantitative measures. The main idea behind our approach is that quality requirements in general have different criticality for software features and thus, must also be tailored and individually specified with appropriate thresholds for each software feature. Using our DSL, not only the acquisition of these measure from external sources in DevOps can be defined, but also their filtering, preprocessing, and evaluation using different time filters, time series operations, and comparison operators. 

Also, we introduced two novel language elements to define the aggregation of evaluation results. When conceptualizing these two language elements and their typical usage scenarios, we incorporated our findings from a previous interview study in which the participants addressed the need for these language capabilities. For specifying results aggregation, we distinguish between quality ratings and quality gates. The former summarize the evaluation results of each software feature based on the average of these evaluation results on a five-point ordinal grading scheme from A-E. Likewise, the latter use these quality ratings to reflect the fitness of individual features or the overall software product through pass, fail, or warning states. Each degree of fulfillment of quality ratings and gates can be described using the DSL. Quality ratings can also demand the fulfillment of individual constraints or particular grades of subordinate quality ratings. Similarly, quality gates can also demand that a software feature reaches a certain grade of quality rating.

Future work needs to concentrate on empirical validations regarding the suitability of the novel two language elements. This particularly pertains to the expressiveness and completeness of the language to formulate conditions for the individual grades of quality ratings and to define the different states of quality gates. Also, methodological and tool support shall be improved to better support engineering teams in defining feature-level quality constraints, quality ratings and gates. Methodological support shall specially cover the elicitation of quality requirements and their individual feature-dependent relevance from the different stakeholders in DevOps, based on the domain of the software product.

==> Revision1/constraint_language.tex <==
%!TEX root = manuscript.tex
\label{constraint_language}
As already stated, the TAICOS approach allows to decompose quality-related stakeholder interests into feature-level quality requirements and specify them in an operational manner as feature constraints. Thereby, each feature constraint utilizes a specific \textit{measure} that is operationalized through an \textit{instrument} and accessed in the constraint declaration by a \textit{variable}. As an example, we could utilize the cyclomatic complexity as a measure of the maintainability of the software. This measure can be directly acquired, e.g., from the \dslkeyword{Sonar} instrument\footnote{https://www.sonarqube.org/} which queries this measure from the corresponding code quality server and assign the value to a variable. The concrete feature-level requirement towards the maintainability and thus, the permissible feature-dependent threshold for this variable, is then expressed as a feature constraint. To evaluate the development of a measure over time, the TAICOS DSL also provides time filters and time series operations. For instance, in the given example one can demand that the average cyclomatic complexity during the last month must be below a certain threshold. Conceptually, variables can hold metrical values (e.g., the number of rule violations or concrete metrics), or ordinal values such as quantiles resulting from benchmarking rule violations with other projects.


\subsection{Grammar and Language Elements}
\label{warningThreshold}
In general, each TAICOS model consists of a project-specific metadata block and the four blocks for specifying measurements and constraints: \dslkeyword{<Interests>}, \dslkeyword{<Features>}, \dslkeyword{<Variables>}, and a list of \dslkeyword{<Constraint>}. 

The metadata block specifies the unique project identifier (\dslkeyword{projectId}) and the  \dslkeyword{<WarningThreshold>}. This threshold denotes the limit in percent below which the user shall be warned in advance, e.g., on a user interface, of possible constraint violations.  
\begin{figure}
\lstset{style=atg,basicstyle=\footnotesize\ttfamily,caption={Grammar rules for defining TAICOS model metadata.},captionpos=b,label=lst:metadata}
\begin{lstlisting}
"projectId: " projectId "." .
<WarningThreshold> ::= "at warning" warningThreshold 
    "before constraint violation." . 
\end{lstlisting}
\end{figure}
Listing \ref{lst:metadata} shows the grammar rules for the model metadata block using the DSL. In listings of grammar rules, I highlight \dslkeyword{<non-terminal symbols>} of the language in angle brackets and \dslkeyword{terminal symbols} without brackets. 
\subsubsection{Variables and Instruments}
\label{variabledefinition}
\label{instrumentdefinition}
A \dslkeyword{<Variable>} defines a name for a concrete measure, its type, and also its acquisition from an \dslkeyword{<Instrument>}. The name of a variable can be arbitrarily chosen and can be used in arbitrary constraints. The language allows three types of variables: \dslkeyword{measure} for numerical metrics, \dslkeyword{rule} for the number of rule violations, and \dslkeyword{rating} for 1-letter quality ratings on an ordinal scale from A to E. The type of a variable also imposes restrictions on the use of the \dslkeyword{comparison} operator, as only variables of the same type can be compared. 

\begin{figure}[h!]
\lstset{style=atg,basicstyle=\footnotesize\ttfamily,caption={Grammar rules for defining variables and instruments.},captionpos=b,label=lst:variablesinstrument}
\begin{lstlisting}
<Variables> ::= "@variables: {"  
    <Variable> { <Variable> } "}." .
<Variable> ::= variable 
    "as" type "from" <Instrument> "." .
type := "measure" | "rule" | "rating" .
<Instrument> ::= instrumentId  
    "(" key ["," param] ")." .
\end{lstlisting}
\end{figure}

An \dslkeyword{Instrument} defines for each variable how it can actually be retrieved from a specific external system. Also, the set of instruments can easily be extended by implementing a specific software interface to integrate further external system for retrieving measures. One could, e.g., declare a variable  \dslkeyword{cyclomaticComplexity as measure from Sonar("complexity")}. This expresses that the metrical variable \linebreak \dslkeyword{cyclomaticComplexity} is acquired from the \dslkeyword{Sonar} instrument, which accesses it using the key \dslkeyword{complexity}. Thereby, the \dslkeyword{key} used by the instrument is predetermined by the external system that the instrument connects to.

\subsubsection{Features} 
\label{featuredefinition}
The \dslkeyword{<Feature>} element specifies a software feature through a unique \dslkeyword{featureId} and a list of contexts each with an individual \dslkeyword{contextId}. In DevOps, quality-related data need to be acquired from different systems, e.g., code repositories, bug databases, application monitoring systems, etc. As features are represented differently by these systems one needs to specify how to identify a feature individually for each system (context). Context-specific metadata are defined for each feature through \dslkeyword{key}-\dslkeyword{value} pairs (see Listing \ref{lst:features}).

\begin{figure}[h!]
\lstset{style=atg,basicstyle=\footnotesize\ttfamily,caption={Grammar rules for defining feature metadata.},captionpos=b,label=lst:features}
\begin{lstlisting}
<Features> ::= "@features: {" 
    <Feature> { <Feature> } "}." .
<Feature> ::= featureId ":" 
    ["with quality-rating" ratingId 
        ["and quality-gate" gateId]
    ]
    ["with quality-gate" gateId ]
    {"context" contextId "with {" 
            { key value "." } 
        "}" 
    }"." .
\end{lstlisting}
\end{figure}
As an example, one could declare a context \textit{filesystem} to denote the source code location of the software feature on the developer's computer, a \textit{git} context to define the repository location of  the versioning system, or an \textit{apm} context to query runtime measures from a system for application performance monitoring. Due to the genericity of this concept, different contexts and thus sources for retrieving feature-dependent quality metrics can be declared. 

\subsubsection{Constraints}
\label{typeofconstraints}
\begin{figure}
\lstset{style=atg,basicstyle=\footnotesize\ttfamily,caption={Grammar rules for defining feature constraints.},captionpos=b,label=lst:featureconstraints}
\begin{lstlisting}
<Constraint> ::= interestId ": {" 
    featureId ": {" <ConstraintBody> 
    {"," <ConstraintBody> } ["as" constraintName] "}." .
<ConstraintBody> ::= 
    ( variable [".benchmark"] ) | 
    ( operation "(" variable "," filter ")" )
    comparison constraintThreshold "." .
operation ::= "min" | "max" | "median" | "avg" | "gradient".
filter ::= "seconds" | "minutes" | "hours" | "days" | "months".
comparison ::= ">" | "<" | "==" | ">=" | "<=".
\end{lstlisting}
\end{figure}
A \dslkeyword{<Constraint>} specifies a quantitative requirement for a criterion, e.g., cyclomatic complexity. The evaluation criteria are expressed in the \dslkeyword{<ConstraintBody>}. Optionally, a constraint can be given a unique \dslkeyword{constraintName} to reference it in definitions of quality ratings (cf. Section \ref{aggregation_language}).
Listing \ref{lst:featureconstraints} shows the grammar rules for feature constraints using time series operations, time filters, and comparison operators. Basically, one can differentiate three variants of constraints: 
\begin{enumerate}
	\item Constraints comparing the most recent value of a variable with a threshold. This is the simplest form of a constraint and works with any type of variable. For instance, one could declare a constraint such as \dslkeyword{video: cyclomaticComplexity < 8} to require that cyclomatic complexity for the software feature \dslkeyword{video} is lower than 8. In this constraint variant, the \dslkeyword{threshold} element can  take metrical values, e.g., the expected cyclomatic complexity or the permissible number of rule violations, or ordinal values expressed as single characters from A to E. 

	\item Constraints utilizing benchmark results of rule violations to evaluate if they lie within a specific quartile of the benchmark base. This type of constraint requires a variable of type \dslkeyword{rule} and is declared by appending \dslkeyword{.benchmark} to the variable name. One could, e.g., declare a variable \dslkeyword{undocumentedMethods as rule from Sonar("squid:UndocumentedApi")} to hold the number of violations of the rule to document public methods. The constraint \dslkeyword{video: undocumentedMethods.benchmark < Q50} would then require that the number of rule violations in the \dslkeyword{video} feature is lower than in 50\% of the benchmarked projects. Thereby, the \dslkeyword{threshold} can take any of the four quartiles which are referred to as \dslkeyword{Q25}, \dslkeyword{Q50}, \dslkeyword{Q75}, and \dslkeyword{Q100}. 

	\item Constraints comparing the result of a time series operation, applied onto measures, with a concrete threshold.  Such constraints can only be expressed for metrical variables, i.e., of type \dslkeyword{measure} or \dslkeyword{rule}. They require a concrete time series \dslkeyword{operation} and a time \dslkeyword{filter} to be specified in the constraint. The constraint \dslkeyword{video: avg(cyclomaticComplexity, days(7)) < 12} defines that the average cyclomatic complexity of the \dslkeyword{video} feature must not have been greater than or equal 12 during the last 7 days. Thereby, the \dslkeyword{threshold} can only take metrical values as the mathematical operations underlying the time series operations are only defined for real numbers. 
\end{enumerate}

In general, threshold values are always given without unit of measurement as this would require conversion between the units of variable and threshold values. Thus, the unit of measurement used for comparison is determined by the instrument that operationalizes the corresponding variable.

\subsubsection{Interests}
Value expectations that shall be regarded by all software features are specified through an \dslkeyword{<Interest>} element with a unique \dslkeyword{interestId} and a textual \dslkeyword{interestDescription} of the objective (see Listing \ref{lst:interests}). Interests can be nested into each other, for example to refine one larger interest into several smaller ones. In that case, the overarching large interest is referred to as \textit{interest group}. 
\begin{figure}[h!]
\lstset{style=atg,basicstyle=\footnotesize\ttfamily,caption={Grammar rules for defining stakeholder interests.},captionpos=b,label=lst:interests}
\begin{lstlisting}
<Interests> ::= "@interests: {" 
    <Interest> { <Interest> } "}." .
<Interest> :: = interestId 
    ["with quality-rating" ratingId] ":" 
    interestDescription ".".
\end{lstlisting}
\end{figure}
For each interest group and interest, a quality rating can be defined that summarizes the evaluation results of the constraints specified for this interest.
\subsubsection{Time Series Operations and Filters}
The DSL provides five different time series operations, like the \dslkeyword{min} and \dslkeyword{max} operation to determine minimum and maximum, the \dslkeyword{median} and \dslkeyword{avg} for calculating median and average, and the \dslkeyword{gradient} operation to calculate the incline of the (linear regression) line of a time series of measures. For filtering time series the language provides five filters such as \dslkeyword{seconds}, \dslkeyword{minutes}, \dslkeyword{hours}, \dslkeyword{days}, and \dslkeyword{months} with a numerical parameter indicating the number of time units to go backwards in time. Time series operations are only applicable for variables with a type of \dslkeyword{measure} or \dslkeyword{rule}. Also, the comparison of a variable with a threshold inevitably requires that both values are of the same type.

\subsection{Comparability of Measures in Feature Constraints}
While the syntatic validity of feature constraints formulated by the user is assured by the parser of the  DSL, it cannot check whether the measures used in the constraints are semantically appropriate to be compared. This particularly pertains to the
\begin{itemize}
\item required normalization of quality-related measures to regard the different code bases of features, and 
\item direction of comparison operators and threshold values. 
\end{itemize}
To address the first point, the TAICOS DSL allows to provide optional parameters in the declaration of an \dslkeyword{instrument}. Information required by an instrument for normalization can that thus be passed. For instance, the \dslkeyword{Sonar} instrument used in the previous example can require a parameter \dslkeyword{normalizationBase=loc} to determine that measures of static code analysis shall be normalized based on lines of code or \dslkeyword{normalizationBase=methodCount} to normalize them based on method count.

The second point relates to the semantically appropriate selection of comparison operators. The choice of the semantically correct comparison operator depends on whether the value of the compared metric should be low or high in order to have a positive impact on quality. For instance, while the value of particular metrics shall always be as \textit{low} as possible (e.g., the technical debt) it is nonetheless possible to demand that this value is \textit{higher} than a given threshold and apply the \dslkeyword{>} operator. As the TAICOS DSL parser does not detect such semantic contradictions it is up to the user to select an operator that compares values and metrics from the background of positive impact on the quality objective, and thus stakeholder interest.

==> Revision1/discussion.tex <==
%!TEX root = manuscript.tex
\label{discussion}
For the practical applicability of a DSL for expressing feature-level quality requirements and aggregating the evaluation results, two key factors need to be addressed. First, context-dependent usage patterns of the language might impose specific performance requirements towards software tools implementing the language. These usage patterns are associated, e.g., with different types of quality requirements and can result in some language elements being more frequently used than others. Second, the DSL must be suitable, expressive, and complete from the perspective of practitioners to address quality requirements. Missing important basically expected capabilities towards the language from practitioners, inevitably hinders its practical adoption or leads to complicated and unintended use of language elements.

We analyzed the performance of the different language elements based on 12 releases (over 1 year) of the widely adopted \textit{Elasticsearch}\footnote{https://www.elastic.co/elasticsearch/} search engine in a lab experiment \cite{haindl_operational_2020}. Thereby we used quality measures from static code analysis which are typical for large-scale software products. While performance characteristics in themselves do not depend on the DSL but on the language's software implementation, each time series operation inherently requires particular mathematical operations. The validation showed that even if the time series operations take into account measures of over one year and of more than 800 classes, they finish within 1 millisecond with the \dslkeyword{gradient} operation taking the longest. However, the most time-consuming part during constraint evaluation attributes to the retrieval of the measures, which basically depends on the concrete software implementation of the language. In \cite{haindl_specifying_2020} we presented our case study with practitioners who applied the language to formulate feature constraints for maintainability requirements. In this context, we identified the \dslkeyword{measure} data type as being most frequently used and the \dslkeyword{min}, \dslkeyword{max}, \dslkeyword{median}, and \dslkeyword{avg} time series operations used far more often than the \dslkeyword{gradient} and \dslkeyword{benchmark} operations. 

In contrast to evaluating feature constraints, far less data are required for aggregating evaluation results either as quality ratings or gates. This is due to both quality ratings and gates relying on already calculated evaluation results to thereof calculate the average. Therefore, we can assume that these language elements will not have a significant impact on the overall time to evaluate feature constraints and aggregate their evaluation results.

Specially to facilitate the definition and interpretation of quality ratings in practice, we have followed the widely used 5-level ordinal scale which is also used in the \textit{Sonarqube}\footnote{https://www.sonarqube.org/} suite, for example. We have also taken deliberate care to avoid complexity in the definition of quality ratings and gates. This means that both types of aggregations shall be applicable by people who are less familiar with technical details (product managers, project managers), in contrast to people who define the feature constraints (software engineers, architects). Nonetheless, as also expressed by the participants of our case study \cite{haindl_specifying_2020}, it is important to be able to access evaluation results of individual constraints, interests, or features in the definition of quality ratings and gates. Also, the translation of quality requirements to each individual feature should be done exclusively through feature constraints, since at the higher levels (i.e. interests groups and features) only subordinate evaluation results are aggregated.

\change{Discuss relation between DevOps and the contribution of the DSL for challenges outlined in the related work section.}


==> Revision1/introduction.tex <==
%!TEX root = manuscript.tex
\label{introduction}
In most software projects, quality requirements are approached as cross-cutting concerns on the top-level of the software product and treated without further refinement for individual software features. This, however, neglects that the same quality requirement might manifest differently among individual software features. As an example, maintainability requirements might be higher for those software features that need to be changed more frequently than others, e.g., because they represent core functionality of the software product or differentiate the product from competitors' alternatives.  Likewise, software features that process real-time data will be subjected to stricter performance requirements than features that typically realize background tasks. To permit the specification of individual quality requirements for different software features and the evaluation of these feature-level quality requirements in DevOps, we developed the \textit{TAICOS approach}. 

We already sketched the first results of our operational DSL for formalizing the fulfillment criteria of feature-level quality requirements as feature constraints \cite{haindl_operational_2020}. An operational DSL that allows automated quality assessments in DevOps must permit to specify these feature constraints, the operationalization of metrics used in the constraints, and the suitable aggregation of evaluation results in an operational manner, individually for different features. In addition, such a DSL needs to address two major challenges: First, it must regard the different types of metrics that typically accrue on the systems involved in DevOps and which are necessary to evaluate the respective constraints. Second, as these metrics' measures evolve over time and change frequently, an appropriate DSL also needs to provide capabilities to express the permissible development of a metric in a particular time frame. 

From the viewpoint of operationalizing such a DSL, the lead time for evaluating feature constraints must be minimal even for large-dimensioned features as well as for constraints taking into account a multitude of a metric' measures. This specially affects its application in DevOps which demands fast and frequent feedback cycles covering large data streams originating from multiple different development and operational systems. In \cite{haindl_operational_2020} we also reported on a lab experiment with our then preliminary software prototype focusing on its performance for operationalization, preprocessing, filtering, and calculation of metrics required for constraint evaluation. Resulting from this lab experiment, the operationalization of the metrics has been identified as the most influential factor affecting constraint processing time. The former concept of our approach required operationalizing the metrics from DevOps related systems on-demand during constraint processing, resulting in respective performance impediments during constraint processing. To overcome this limitation, our current concept employs a time-series database to which operationalized metrics are pushed frequently prior to constraint evaluation. 

In \cite{haindl_specifying_2020} we presented our findings from a user study with practitioners to assess the completeness, expressiveness, scope, and suitability of the DSL for specifying maintainability requirements on feature-level as one important software quality aspect. While the participants rated the aforementioned aspects of the DSL with overall high levels, the experts also stressed the necessity of expressing the aggregation of constraint evaluation results. To address this requirement, we extended the DSL by two novel elements that allow to specify the aggregation of constraint evaluation results through \textit{quality ratings} and \textit{quality gates}. As extension of our previous works this paper elaborates the final version of this DSL covering the new language elements for aggregating evaluation results, a metamodel to define the relations between the language elements, and a schematic diagram of the integration of our approach in DevOps. This illustration defines the interaction sequence for each DevOps phase between systems providing relevant metrics and the components of our approach.

The paper is structured as follows: In Section \ref{related_work} we elaborate on the related work in this field and the identified limitations that we address in our contributions. Section \ref{concepts} describes the operationalization and integration of our approach in DevOps, followed by discussing the metamodel of the TAICOS DSL in Section \ref{metamodel}. Subsequently, in Section \ref{constraint_language} we present the DSL elements for specifying feature-level quality constraints, complemented by the presentation of language elements for defining the aggregation of evaluation results on different levels in Section \ref{aggregation_language}. Afterwards, in Section \ref{example} we show visualizations of constraint evaluation results, quality ratings, and gates based on real data of the Telegram mobile app. In Section \ref{discussion} we discuss the presented DSL and particularly the two new language elements for results aggregation in face of the findings from our previous case studies. Finally, we sketch possible directions for future work and conclude our paper in Section \ref{conclusion}. 

==> Revision1/metamodel.tex <==
%!TEX root = manuscript.tex
\label{metamodel}
\change{meta model hier beschreiben. evtl texte aus den beiden nachfolgenden Kapitel hierher verschieben}
\begin{figure}[h]
\centering
\includegraphics[scale=0.42]{images/metamodel.pdf}\caption{Meta model of the TAICOS DSL.\label{fig:meta_model}}
\end{figure}


==> Revision1/prototype.tex <==
%!TEX root = manuscript.tex
\label{prototype}

==> Revision1/related_work.tex <==
%!TEX root = manuscript.tex
\label{related_work}
We separate the related work in this field into four streams of research. The first stream relates to constraint languages for expressing and evaluating the fulfillment of quality requirements. Event-based constraint languages \cite{robinson_monitoring_2002,robinson_roadmap_2010,robinson_requirements_2006} mainly target on monitoring and assuring special runtime requirements of systems, e.g., the proper message exchange and failover in systems-of-systems (SoS). They rely on monitoring \textit{discrete} events and thus are less suitable for monitoring the fulfillment of \textit{continuous} quality requirements, such as e.g., maintainability requirements. Vierhauser et al. describe a DSL-based approach for event monitoring in SoS \cite{vierhauser_developing_2015}. The language allows to define event triggers, conditions, and timing requirements for these conditions. Rosenberg et al. present the \textit{Vienna Composition Language (VCL)} \cite{rosenberg_end--end_2009}, a DSL for QoS-aware web service composition. It permits to specify QoS attributes e.g., response time or availability, for individual services. Lastly, Goknil and Peraldi-Frati developed a DSL that provides dedicated language elements for expressing time spans, jitter, minimum, and maximum of measures \cite{goknil_dsl_2012}.

Domain-specific languages and model-driven approaches for the DevOps context are at the center of the second stream of related research. Colantoni et al. contributed \textit{DevOpsML}, a conceptual framework for modeling and integrating DevOps processes across platforms \cite{colantoni_devopsml_2020}. The interfaces of tools and their provided capabilities are the building blocks of these platforms. In the gist of this paper is the metamodel which relates processes, tools, and platforms in DevOps. The metamodel gives a blueprint to express the most relevant aspects of a real-world DevOps environment. This resembles the approach of Wettinger et al. (\textit{DevOpSlang}) which provides a DSL to define the automation of continuous delivery steps in DevOps \cite{wettinger_devopslang_2014}. Unlike the previously discussed work, this allows an operational definition of continuous delivery steps by means of commands, but is less applicable to other DevOps phases than the approach of Colantoni et al. In their most recent paper, Colantoni et al.  report on their current progress towards a model-driven approaches for continuous consistency checking of DevOps artefacts \cite{colantoni_towards_2021}. It is centered around the \textit{Keptn} framework \cite{dynatrace_keptn_2021} to monitor delivery and operation requirements expressed by \textit{Service Level Indicators (SLI)} \cite{dynatrace_keptn_2021-1} and \textit{Service Level Objectives (SLO)} \cite{dynatrace_keptn_2021-2}. The former defines quantitative measures for a particular service level, the latter concretizes the target values or ranges for the SLI measures. Validation rules for consistency requirements are then formulated based on SLIs and SLOs and their fulfillment checked by the Keptn framework.

Approaches for the aggregation of software quality evaluation results are researched in the third stream of related research addresses. Siavvas et al. present the \textit{QUATCH} framework for software product quality assessment \cite{siavvas_qatch_2017}. In this approach, multiple metric-based quality assessments are summarized in a single score, which is subsequently mapped onto a rating. While the score is a metrical value that lies in the interval between 0 and 1 (with 0 reflecting lower quality), the rating is an ordinal representation of this metrical value. The relation between score and rating is linear, i.e., the higher the score, the higher the rating on its ordinal scale. To reflect the individual importance of the metrics as the basis of the quality score, each metric can be assigned a different weight. The quality score is then calculated from the weighted average of these metrics. Apel et al. elaborate a metric-based quality rating approach for microservice architectures \cite{apel_towards_2019}. In contrast to Siavvas et al., these authors do not calculate a quality rating per se, but examine the suitability of quality metrics relevant for microservice architectures to rate the quality of each of the eight ISO 25010 subcharacteristics. This also follows the idea of summarizing multiple individual metrics into one single quality score, e.g., through building the average of these metrics. A quality rating approach that takes into account threshold values for individual metrics is presented by \cite{bansal_software_2016}. Thereby, to fulfill a certain rating (similar to school grades) individual metrics need to lie within a specific predefined interval. In the remainder of this paper we refer to ``stage gates'' as quality gates, as also the further cited literature uses this term. Flohr examines the appropriateness of criteria used in quality gates to help decide whether quality milestones in projects are fulfilled \cite{flohr_defining_2008}. He concludes that systematic top-down approaches based on software quality models and deriving criteria from abstract business goals are must suitable for the definition of quality gates. However, as these findings originate from a validation through student experiments this might affect the generalizability of these findings. Schermann et al.  report on a case study with companies to examine the benefits of using quality gates for continuous delivery of software projects \cite{schermann_towards_2016}. The case study revealed a relation between the effort companies put into quality gates and the pace with which they can release new versions of their software. In a subsequent work of these authors \cite{schermann_were_2018}, this observation is explained with the intrinsic goal behind continuous delivery to increase velocity. This pertains to the time needed to pass all quality gates and approval steps until the changes to the software reaches the production environment, while at the same time ensuring a high level of software product quality. Deniz gives a concrete example of quality gates that focus on object-oriented design quality based on the metrics suite of Chidamber \& Kemerer for object-oriented design \cite{deniz_software_2015,chidamber_metrics_1994}. It determines one of three states of quality gates (success, warning, fail) based on the number of quality-related rule violations. Each metrics must lie within specific thresholds to reach one of the three states. The overall quality gate of software components is determined by assigning points (100 for success, 50 for warning, 0 for fail), building the average of these points, and determining one of the three states thereof.

Research on the application of quality gates in software projects is covered by the fourth stream of related work. The idea of quality gates goes back to the \textit{stage-gate process} first presented by Cooper \cite{cooper_perspective_1994,cooper_product_1999} to assert the product quality at important transitions between product development phases. At these transition, \textit{stage gates} assess whether the preceding product phase meets particular criteria so that the development can proceed to the next stage. Besides other areas, the idea is applicable also to agile software product development \cite{borba_agile_2019,bianchi_agile_2020} to ensure software quality between sprints. Raatikainen et al. report on an exploratory multiple case study to examine different stages, controlled by gates, in lean software development in startups \cite{raatikainen_eight_2016}. They propose four different stages and respective gates, from ideation to scaling, to ensure the economic viability of the developed software product. A further industrial case study investigated the application of the stage gate concept to agile software development \cite{bianchi_agile_2020}. The authors stress the importance of defining stage gates that take into account metrics from different domains and also the requirement to flexibly adapt these gates, particularly in an agile context. To properly summarize the quality level of each development phase, stage gates shall be composed of metrics particularly relevant for the preceding phase. 

\subsection{Summarization of Limitations}
The main limitations of existing DSLs for evaluating quality requirements in DevOps can be summarized as follows: First, they do not allow to define quality requirements individually for different software features. Second, they are mainly suitable for defining quality requirements that are based on discrete events. Third, other DSLs do not explicitly address the operationalization of the measures required for evaluating the fulfillment of the described requirements on feature-level. Among the previously discussed related approaches, only the SLI concept of Keptn \cite{dynatrace_keptn_2021-1} addresses the operationalization of measures in a generic manner. It however requires to implement the respective API to retrieve the measures prior to their evaluation. Fourth, apart from the Keptn DSL they provide only basic support for time-filtering and time-series analysis of constraint measures. No DSL covered by similar approaches fulfills all requirements for feature-oriented quality evaluation in DevOps (see Section \ref{introduction}, i.e. the definition of metric operationalization from DevOps-related systems, threshold definition on feature-level, support for time-based filtering and time-series operation) but only partial aspects.

Also, as mentioned in Section \ref{related_work}, several approaches exist for defining quality ratings and gates. However, none of these approaches is based on a declarative language and instead is implemented in a project-specific manner. As such it is not possible to adapt the calculation of quality ratings and gates, e.g., to take into account other quality metrics or customize the weight of metrics. Adjusting the weight, for instance, is necessary to reflect the different importance of a metric in the quality score, which is calculated through the weighted average. As also pointed out in \cite{siavvas_qatch_2017}, the recent advent of machine learning approaches for software quality rating yet allows to calculate quality ratings, but in a way that is mostly intransparent and difficult to customize in practice. Further, these approaches do not allow to incorporate domain-knowledge available in the companies to formulate quality gates and ratings.

\subsection{Contributions}
In this paper, we contribute an operational DSL language that addresses the aforementioned limitations. Particularly, as a demarcation to related works in this field, our DSL allows to
\begin{itemize}
	\item specify quality requirements of software features in an operational manner using quantitative metrics and evaluation criteria as feature constraints
	\item define the operationalization of these metrics, i.e., their acquisition from the various DevOps-related
	\item support for time-based filtering and time-series analysis of metrics' measures in feature constraints
	\item specify quality ratings flexibly in different granularity levels based on constraint evaluation results
	\item define quality gates on software feature- and product-level based on fulfillment criteria of quality ratings on different granularity levels
\end{itemize}

Further, we contribute a metamodel of our DSL that defines the relation between the language elements and a schematic diagram showing the integration of the TAICOS approach in DevOps. Both the metamodel and the schematic diagram shall facilitate the development of software extensions, e.g., further connectors to external systems and language elements, and their operational integration into a real-world DevOps environment.




==> Revision1/threats.tex <==
%!TEX root = manuscript.tex

==> case_study.tex <==
%!TEX root = manuscript.tex
\label{case_study}
\subsection{Software Prototype}
\subsection{Scope and Expressiveness of DSL elements}

==> prototype.tex <==
%!TEX root = manuscript.tex
\label{prototype}

==> threats.tex <==
%!TEX root = manuscript.tex
